Gaseous Galaxy Halos

Galactic halo gas traces inflowing star formation fuel and feedback from a galaxy's disk and is therefore crucial to our understanding of galaxy evolution. In this review, we summarize the multi-wavelength observational properties and origin models of Galactic and low redshift spiral galaxy halo gas. Galactic halos contain multiphase gas flows that are dominated in mass by the ionized component and extend to large radii. The densest, coldest halo gas observed in neutral hydrogen (HI) is generally closest to the disk (< 20 kpc), and absorption line results indicate warm and warm-hot diffuse halo gas is present throughout a galaxy's halo. The hot halo gas detected is not a significant fraction of a galaxy's baryons. The disk-halo interface is where the multiphase flows are integrated into the star forming disk, and there is evidence for both feedback and fueling at this interface from the temperature and kinematic gradient of the gas and HI structures. The origin and fate of halo gas is considered in the context of cosmological and idealized local simulations. Accretion along cosmic filaments occurs in both a hot (> 10^5.5 K) and cold mode in simulations, with the compressed material close to the disk the coldest and densest, in agreement with observations. There is evidence in halo gas observations for radiative and mechanical feedback mechanisms, including escaping photons from the disk, supernova-driven winds, and a galactic fountain. Satellite accretion also leaves behind abundant halo gas. This satellite gas interacts with the existing halo medium, and much of this gas will become part of the diffuse halo before it can reach the disk. The accretion rate from cold and warm halo gas is generally below a galaxy disk's star formation rate, but gas at the disk-halo interface and stellar feedback may be important additional fuel sources.

==> views.tex <==
 VIEW={Overview}
  COO=5.985597133636475 6.663844108581543 -5.449902534484863
  C2C=0.8753247857093811 0.035229478031396866 0.482250452041626
  ROO=43.90569672694108
  ROLL=-2.7539388900949
  AAC=60.000001669652114
  BGCOLOR=0.894118 0.827451 0.737255
  LIGHTS=CAD
  RENDERMODE=Solid
    PART={Disk}
    VISIBLE=true
  END
  PART={Bulge}
    VISIBLE=true
  END
  PART={Sun}
    VISIBLE=true
  END
END
VIEW={Complex C [Celestial]}
  COO=8.383414268493652 -3.5624449253082275 2.7557156085968018
  C2C=0.02587692253291607 0.7907066345214844 -0.6116480827331543
  ROO=4.505393928130129
  AAC=90.00000250447816
  BGCOLOR=0.894118 0.827451 0.737255
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Disk}
    VISIBLE=false
  END
  PART={Bulge}
    VISIBLE=false
  END
  PART={Sun}
    VISIBLE=false
  END
END
VIEW={Magellanic Stream [Celestial]}
  COO=-0.9859270453453064 7.980239391326904 -37.16588592529297
  C2C=0.24211949110031128 -0.20368820428848267 0.9486249089241028
  ROO=39.17869437300632
  AAC=90.00000250447816
  BGCOLOR=0.894118 0.827451 0.737255
  LIGHTS=CAD
  RENDERMODE=Solid
  PART={Disk}
    VISIBLE=false
  END
  PART={Bulge}
    VISIBLE=false
  END
  PART={Sun}
    VISIBLE=false
  END
END
VIEW={Complex C [Physical]}
  COO=9.212745666503906 -0.5792254209518433 4.477636337280273
  C2C=0.28651753067970276 0.9261650443077087 0.24520619213581085
  ROO=11.400171619930429
  AAC=60.000001669652114
  BGCOLOR=0.894118 0.827451 0.737255
  LIGHTS=CAD
  RENDERMODE=Solid
END
VIEW={Magellanic Stream [Physical]}
  COO=-5.218128681182861 -11.46090030670166 -32.42790222167969
  C2C=0.9046380519866943 0.37012943625450134 0.211268350481987
  ROO=140.69519775697748
  AAC=60.000001669652114
  BGCOLOR=0.894118 0.827451 0.737255
  LIGHTS=CAD
  RENDERMODE=Solid
END


